Synthesis of Distributed Agreement-Based Systems with Efficiently-Decidable Verification (Extended Version)

Distributed agreement-based (DAB) systems use common distributed agreement protocols such as leader election and consensus as building blocks for their target functionality. While automated verification for DAB systems is undecidable in general, recent work identifies a large class of DAB systems for which verification is efficiently-decidable. Unfortunately, the conditions characterizing such a class can be opaque and non-intuitive, and can pose a significant challenge to system designers trying to model their systems in this class. In this paper, we present a synthesis-driven tool, Cinnabar, to help system designers building DAB systems "fit" their intended designs into an efficiently-decidable class. In particular, starting from an initial sketch provided by the designer, Cinnabar generates sketch completions using a counterexample-guided procedure. The core technique relies on a compact encoding of a set of related counterexamples. We demonstrate Cinnabar's effectiveness by successfully and efficiently synthesizing completions for a variety of interesting DAB systems.

==> algorithm-backup.tex <==
\section{Problem Definition and Solution Approach}
\label{sec:algorithm} 
%\nour{this section is currently written for the ``instantiation'' of the approach. If we settle on posing the paper as a general approach with an instantiation to our case, we can adjust accordingly.\\}

In this section, we define the parameterized synthesis problem for distributed agreement-based systems modeled in \aml as well as our CEGIS-based approach to solving it. 

\begin{definition} [\aml Parameterized Synthesis Problem (\mpsp)]
Given a \aml program sketch $\psketch$ with a set of uninterpreted functions $\uFuns$, an environment process $\p_e$, and \permissible safety specifications $\safetySpec$, find an interpretation $\interpretation \in \interpretations$ to obtain a \aml program $\pcomplete 
%\coloneq \interpretation(\psketch)
$ with a corresponding global semantics $\iglobalSemantics(n) \coloneqq {\pcomplete}_1 || \ldots || {\pcomplete}_n || \p_e$ such that $\forall n: \iglobalSemantics(n) \models \safetySpec$. %\editt{see the commented, more-nuanced version}
\end{definition} 
%
%\nour{This is the more-nuanced version. I like the first version better as it's a more classical problem definition. The latter ``hints'' into how we solve this problem, which may or may not be what we want.}
%
%\begin{definition} [\aml Parameterized Synthesis Problem (\mpsp)]
%Given a \aml program sketch $\psketch$ with a set of uninterpreted functions $\uFuns$, an environment process $\p_e$, \permissible safety specifications $\safetySpec$, and liveness specifications $\livenessSpec$, find an interpretation $\interpretation \in \interpretations$ to obtain a \aml program $\pcomplete 
%%\coloneq \interpretation(\psketch)
%$ with a corresponding local semantics $\isemantics$ and global semantics $\globalSemantics_\interpretation(n) \coloneqq {\pcomplete}_1 || \ldots || {\pcomplete}_n || \p_e$ such that:
%\begin{compactenum}
%%\item $\pcomplete$ is \chwellbehaved and \amenable with cutoff value $c$,
%\item $\isemantics$ is \chwellbehaved,
%\item $\isemantics$ is \amenable with cutoff value $c$,
%\item $\globalSemantics_\interpretation(c) \models \safetySpecc$, and,
%\item $\globalSemantics_\interpretation(c) \models \livenessSpec$.
%\end{compactenum}
%
%\end{definition}
\begin{figure}[b]
\includegraphics[width=0.9\linewidth]{flow.pdf}
\caption{Overview of the multi-stage CEGIS Loop in \tool.}
% In the figure, $pc$ and $ca$ are short for \chwellbehavedness and \amenability, respectively.
%}
\label{fig:flow}
\end{figure}
%\nour{highlight parameterized safty vs liveness}

To solve the \mpsp, 
%we present 
\tool
%, a parameterized synthesis framework built with 
adopts the multi-stage, CEGIS-based architecture shown in \figref{flow}. We now define the main components of \tool, provide an algorithm describing how it works, then reason about the correctness of the algorithm. 
\begin{itemize}
\item A \textsc{Teacher}, based on 
%\cite{Jaber.QuickSilver.OOSLA.2021} 
%is a \teacher for 
\kinarach, a verifier for
agreement-based distributed systems modeled in \aml capable of checking \chwellbehavedness and \amenability conditions. %As discussed in \secref{sketches}, we extend \kinarach to accept process sketches and keep track of disabled local transitions in the local semantics.  
\item A \textsc{Learner}, denoted $\learnerSymbol$, based on the Z3 SMT Solver \cite{z3} that provides interpretations from the set of all interpretations, $\interpretations$. The \learner $\learnerSymbol$ accepts a set $\constraints$ of \emph{constraints} over the uninterpreted functions $\uFuns$ and ensures that any interpretation $\interpretation$ it provides satisfies these constraints (i.e., $\interpretation \models \constraints$). A constraint $\constraint \in \constraints$ is a well-typed Boolean formula over uninterpreted function applications and values in the corresponding functions' return types. Effectively, every constraint the \learner receives serves as a ``hint'' on what the correct interpretation should be. Note that if the \learner runs out of interpretations to provide, then the synthesis procedure has failed. %Note that the oracle $\oracle$ is only aware of the uninterpreted functions $\uFuns$,  %\editt{e.g., $f_a(1,2)>3 \land f_b(1) \neq f_c(2,7)$}
\item The \code{complete} component that simply obtains a candidate process $\pcomplete$ from the provided process sketch $\psketch$ by replacing every uninterpreted function $\uFun \in \uFuns$ in $\psketch$ with its function interpretation $\interpretation(\uFun)$ according to the interpretation $\interpretation$ provided by the \learner.

\item The \code{extract} components are used to extract an \emph{explanation}, denoted $\cex$, \neww{if 
%the \teacher
\kinarach fails at any stage.} 
Such a $\cex$ indicates the \emph{root-cause} for \emph{why} a given condition did not hold. We expand of the \counterexample extraction techniques in \secref{extraction}.
%Note that such extraction strategies depend on the properties that fail. 
%The \code{extract} components provide \emph{counter-examples} that show the failure of a given property.
\item The \code{encode} component provides a \emph{uniform} encoding that distills the various 
\counterexamples provided by the \counterexample extraction components to a constraint $\constraint$ that is added to the \learner $\learnerSymbol$. An encoding of some counter example $\cex$ ensures that \emph{any} interpretation provided by $\learnerSymbol$ will not exhibit a similar violation to that captured by $\cex$. We expand on the encoding procedure in \secref{encoding}.
\end{itemize}

\tool's approach to solving \mpsp is presented in \algoref{synthAlgo}. On a high-level, the algorithm is designed so that the first two stages check \chwellbehavedness and \amenability which ensures that the candidate program is in the \effdecidable fragment of \aml. Then, it proceeds to the latter two stages where it computes a cutoff value, and check if the cutoff-sized system is safe and live.

More precisely, we start with an empty set of constraints, $\constraints$ (\lineref{emptyconstraints}) over the set $\uFuns$ of uninterpreted functions in the process sketch $\psketch$.
At each iteration of the CEGIS loop, we obtain an interpretation $\interpretation$ of the uninterpreted functions that satisfies all the constraints collected so far (\lineref{interpret}). 
Then, if such interpretation exists, we use that interpretation to obtain the candidate process $\pcomplete$ (\lineref{completed}). 
Then, we check if the system described the process $\pcomplete$ is \chwellbehaved, \amenable, safe, and live. At any stage, if the process fails any of these checks, we extract the root-cause of the failure, encode a constraint ruling out that failure, add the constraint to the \learner, and start over. For instance, we check if $\pcomplete$ is \chwellbehaved (\lineref{compatibility}) and if it is not (\lineref{notcompatible}) we encode the extracted \counterexample $\cexPhComp$ as a constraint, add it to the overall set of constraints (\lineref{encodeph}), and start over (\lineref{startoverp}). 

Note that \tool utilizes various \counterexample extractions at each stage. Such open-box approach allows for more-targeted \counterexample extractions that utilize domain-specific knowledge. Finally, we show that the described procedure (\algoref{synthAlgo}) is sound and complete.

\begin{lemma}
\label{lem:sound}
The synthesis procedure proposed in \algoref{synthAlgo} to solve the \mpsp is sound and complete. \end{lemma}
\noindent{\em Proof.}
The soundness of the procedure follows directly from the soundness of \kinarach, shown in \cite{Jaber.QuickSilver.OOSLA.2021}. In particular, The first two stages ensure that the \aml Parameterized Verification Problem is decidable for the candidate process $\pcomplete$ and that $c$ is valid cutoff (i.e., $\iglobalSemantics(c) \models \safetySpecc \Leftrightarrow \forall n:\iglobalSemantics(n) \models \safetySpec$). Stage three ensures that the cutoff-seized system is indeed correct (i.e., $\iglobalSemantics(c) \models \safetySpecc$). The last stage to check liveness merely filters out trivial solutions and hence, has no effect on soundness.

%\begin{lemma}
%\label{lem:complete}
%The synthesis procedure proposed in \algoref{synthAlgo} is complete. \end{lemma}
%\noindent{\em Proof.} 
The completeness of the synthesis procedure hinges on the set of all interpretations $\interpretations$ being finite. Then, the loop will either terminate with a correct candidate process $\pcomplete$, or exhaust all possible interpretations and terminate with \code{null}. Since (i) we allow a finite number of uninterpreted functions in a program sketch $\psketch$, (ii) each function is over finite-domain local variables, and (iii) there are a finite number of local variables in $\psketch$, the set $\interpretations$ is finite and termination is guaranteed.
%
%\edit{Define the parts here}
%\edit{For the oracle, add this:}
%\begin{compactenum}
%\item $\constraint$ be a constraint represented as a well-typed Boolean formula over function application expressions and values in the corresponding functions' return types. \editt{e.g., $f_a(1,2)>3 \land f_b(1) \neq f_c(2,7)$}
%\item $\allConstraints$ is the set of all such constraints $\constraint$.
%\item $\oracle$ be an oracle that accepts a set $\constraints \subseteq \allConstraints$ of constraints and yields an interpretation $\interpretation \in \interpretations$ such that the $\interpretation \models \constraints$. 
%\end{compactenum}
%
%
%\edit{for liveness, say that we need to rule out trivial solutions}


\input{synthesisAlgorithm}

%
%\begin{figure}
%\includegraphics[width=\linewidth]{flow.jpg}
%\caption{Overview of the CEGIS Loop.}
%\label{fig:flow}
%\end{figure}
%

%\edit{add the figure}
%\edit{In the next section: define the interfaces and the types}
%\edit{In the next section: define the calls encode and induce}



==> choosemodel-old.tex <==
\subsection{OLD Semantics of \aml programs with \Aevents}
\label{sec:choosemodelx}

\swen{subsection title and intro have to be revised}
%- 3.1: Point C2: this seems a bit circular: defines consistent via consistent.
%Can you define what exactly "globally consistent" means? The local results are
%all the same? Then say that.

\Consprot protocols and, more broadly, {\em distributed agreement} protocols
such as leader election, $k$-set agreement~\cite{chaudhuri1990agreement},
Paxos~\cite{lamport1998part} and Multi-Paxos~\cite{chandra2007paxos} enable
their participants to collectively decide on a set of {\em proposals} in a
distributed setting. 
%\roopsha{Reword/expand the following}
%Many different strategies exist to implement this.
%%~\cite{lamport1998part,chandra2007paxos,ongaro2014search,shapiro2011conflict}.
%For example,
%every value may be agreed on separately (e.g. Paxos~\cite{lamport1998part}). Or, a
%participant may be picked as leader (e.g. Multi-Paxos~\cite{chandra2007paxos}, 
%Raft~\cite{ongaro2014search}), and then that leader decides the values for all other
%participants. %Or, participants may have a baked-in fixed strategy to locally
%%pick a value from a set of conflicting values (e.g.
%%CRDTs~\cite{shapiro2011conflict}). 
While there are many different strategies for distributed agreement, 
any distributed agreement protocol boils down
to selecting a set of \emph{winning proposals} 
in a globally consistent way from a
set of proposals provided by the \emph{participants}.
Breaking this down further, any correct agreement protocol implementation satisfies
the following precondition and postcondition.
\begin{compactenum}[C1]
\item {\em Consistent Participants Precondition}. The agreement round 
  starts when all participating processes  
  agree on {\em with whom} to invoke the protocol.\footnote{Note that 
  systems in which \emph{all} processes intend to participate in the
agreement round (e.g., all servers trying to elect a leader) trivially satisfy
C1.  The more general form of the precondition C1 is to enable systems to
invoke agreement rounds with only a subset of processes (e.g., in \figref{satsfig},
only aircraft in the \st{Enter} zone participate in the agreement round leading to the \st{HoldLeft} and \st{HoldRight} zones \swen{needs to fit the new presentation of the example}).}
\item {\em Consistent Winners Postcondition}. When
the agreement round ends, all participants agree on the set of winning proposals. 
\end{compactenum}
%Note that all systems in which processes begin with knowledge of all other
%process indices trivially satisfy C1. We merely extend this precondition to
%allow processes to narrow this universal participants list in a consistent way
%to achieve another consitent participants list. This may be done with
%\consagree, or with some less-sophisticated mechanism (e.g. selecting the
%$\chcard$ lowest processes indices).
Thus, to encapsulate rounds of
agreement, the \ch model extends the basic model from \secref{basicmodel} with
a special {\em atomic} global transition, denoted $\chgt$, that comes with a
specification of expected behavior, expressed as the precondition-postcondition
pair (C1,C2).
%\nour{a footnote introducing agreement/validity/termination here sounds more fitting that 3 pages later.}
We make this more precise in what follows.
%\edit{Sometimes we talk about \ch are \emph{one} non-deterministic transition
%VS a set of transitions where with guard true (hence the choice among them is
%nondeterministic). I will mark all places we talk about this by chStyle.}

\edit{Justify the two conditions using Agreement, validity, and termination? Proof sketch that these conditions imply C1 and C2?}

% 0. todo
%\edit{define $s.loc$  and $s.val(v) in 2.1$:
%$s.loc$ denotes the location $\q$ in local state $s$, 
% the notation 
%$\gq[i].val(\chvar)$ denotes the value of $\chvar$ in state $\gq[i]$.
%}
% 1. define the round and its goal

\swen{need to connect earlier to AML(?)}

Let us fix a round of agreement
with \emph{participants} $\chset \subseteq \Ind$, \emph{cardinality} $\chcard$
(corresponding to the number of proposals to be agreed upon), \swen{do we need to make clear that the following are local variables of each process?} {\em proposal
  variable} $\chvar$ on whose value(s) the participants wish to agree, and
\emph{agreement variable} $\winvar$ where each participant expects the results
of \consagree to be available.  We model this agreement round with a
nondeterministic, atomic global $\chgt$ transition from a \gcs state that satisfies precondition C1 to a set of \gce states, each satisfying
postcondition C2.  In what follows, we characterize such global states, and
show how to abstract various \consagree protocols using \ch transitions.\\
 
% 3. mention stuff needed for GlobalAgreementStart
% 4. how to define GlobalAgreementStart states

\para{Identifying GlobalAgreementStart States.} For this round of agreement,
let $\chlocs \subseteq \Q$ be the set of locations from which the
participating processes in this agreement round may begin the round.
%(i.e. are in locations with matching \code{\PartitionCons} or \code{\ValueCons} handlers).
A global state is a \gcs state, $\gqs$, if there exists a set $\chset$ 
of processes
that are in such  locations $\chlocs$ \emph{and} have consistent participant
sets --- essentially satisfying condition C1. Formally, 
\begin{compactenum}[(1)]
\item $\forall i \in \chset : {\gqs}[i].loc \in \chlocs$, and,%= \chloc_i \in \chlocs$,
\item $\forall i,j \in \chset : (S_i =S_j)$,
\end{compactenum}
where $q[i]$ denotes the local state of process $P_i$ in global state $q$ and
$S_i$ denotes the local set of participants\footnote{We place no restrictions on how
  these sets are constructed. While such sets are usually predefined, we allow
  more flexibility by permitting processes to exchange messages to construct
  them.} constructed by process $P_i$. 

%The state $\gcs$ represents the global state in the system where
%processes are ready to start \consagree.

% 5. stuff needed for GlobalAgreementEnd states
% 6. defining the state itself
 %Next, we need to identify all the possible \gce states where \consagree has been reached. 

 While practical \consagree protocols share precondition C1, they have slightly
 different objectives. For instance, Paxos~\cite{lamport1998part} aims to
 achieve \consagree over a value while a leader election protocol aims to
 \emph{partition} the participants into leaders and followers. In order to
 capture such differences, we carefully design our \ch transitions to enable
 \consagree on a set of values as well as the ability to partition the
 participants into ``winners'' and ``losers''. This is reflected in the way we
 characterize \gce states below.\\

%Once a valid $\gqs$ state is identified, we need to identify \gce states to capture 
%the objectives of practical \consagree protocols. Such objectives vary depending on the protocol at hand. For instance, Paxos~\cite{lamport1998part} aims to achieve \consagree over a value while a Leader Election protocol aims to \emph{partition} the participants into leaders and followers. In order to subsume various \consagree protocols, we carefully design our \ch transitions to enable \consagree on a set of values as well as the ability to partition the participants into ``winners'' and ``losers'' %This is reflected in the way we characterize \gce states, 
%as we shall see.\\

\para{Identifying GlobalAgreementEnd States.} Once a valid $\gqs$ state is
identified, each participant $P_i$ submits a proposal $\proposal{i} =
(i,\gqs[i].val(\chvar))$, consisting of the proposing process's
index and the value it proposes from its proposal variable $\chvar$.  Let
$\winset^*$ denote the set of all $k$-sized sets of proposals 
(i.e., sets of 
proposals that may ``win'' the round)
and let $\winset \in \winset^*$ denote a set of such winning proposals.
Additionally, let $w_i$ ($l_i$, resp.) denote the location to which $P_i$
transitions when $\proposal{i} \in \winset$ ($\proposal{i} \not \in \winset$, resp.).
For each $\winset \in \winset^*$, we identify a \gce
state, $\gqe^\winset$, satisfying condition C2 as follows:
%\footnote{The set $\winset^*$ is constructed as follows. Let 
%$\Psi \coloneqq\{\proposal{i} \mid i \in \chset\}$  be the set of all proposals submitted by the participants. Then, $\winset^* \coloneqq \{\winset \in \powerset(\Psi) \mid \, |\winset| = \chcard\}$ is the set of all possible sets of winning proposals}. 

%In order to allow every possible outcome of the \consagree protocol, we add a \ch transition from $\gqs$ (defined above) to every \gce state $\gqe^\winset$ (corresponding to
\begin{compactenum}[(1)]
\item $\forall i \in \chset: \; \proposal{i} \in \winset \;  \implies\;  \gqe^\winset[i].loc = w_i$,
\item $\forall i \in \chset: \; \proposal{i} \not \in \winset \;  \implies\;  \gqe^\winset[i].loc = l_i$,
\item $\forall i \in \chset: \; \gqe^\winset[i].val(\winvar) = \winset$,
\item $\forall i \in \Ind \setminus \chset: \gqe^\winset[i] = \gqs[i]$.
\end{compactenum}
Thus, in any possible $\gqe^\winset$, the location of 
each participating process $P_i$ is
updated to $w_i$ or $l_i$ \emph{and} the value of the agreement variable 
$\winvar$ is updated with the results of  
\consagree.\\

\para{Various \Consagree Protocols as \ch Transitions.} %So far, we illustrated \mn{\swen{something is wrong here}} how \consagree can be abstracted into a set of \ch transitions. We note that
We demonstrate the utility of the \llm in capturing different real-world
\consagree protocols with \ch transitions. We consider two variants of
agreement: \emph{\valstore} and \emph{\wam}.  \Valstore \consagree can model
protocols like Paxos~\cite{lamport1998part} and $k$-set
agreement~\cite{chaudhuri1990agreement} which target agreement on (a set of)
values without necessarily distinguishing between the ``winning processes'' and
``losing processes''; to enable parameterized reasoning over systems in the
\llm, we restrict the domain of such values to be finite.  On the other hand,
\wam \consagree can model variants of leader election protocols which partition
the participants into winning processes and losing processes and are not
typically concerned with variable valuations; to partition an {\em unbounded}
number of processes, \wam involves transitioning participants into a
\emph{finite} number of distinct locations in a process definition.

% Done 1. Highlight process-local versions and differences (destination locations)\\
% Done 2. Introduce process-local notation for later use. 
%3. Highlight global versions and differences (variable valuations and locations)\\

In a process definition, we denote a round of \valstore \consagree with a $\winvar = $ \code{\ValueCons} $(\chset, \chcard, \chvar)$ handler which corresponds to a local transition $\trans{c}{\chfig(\chset, \chcard,\chvar,\winvar)}{d}$.
All participants start in a location $c$ with their proposals stored in variable $\chvar$, and the \consagree round ends with all participants moving to a location $d$ with the result of the \consagree in their variable $\winvar$.
%Observe that in \valstore \consagree, all participating processes move to a single location, which we denote $d$, because the result of \consagree is stored within the variable $\winvar$.
In contrast, we denote a round of \wam \consagree with \code{\PartitionCons}$(\chset, \chcard)$ handlers which correspond to two local transitions: $\trans{c}{\chfig(\chset, \chcard)}{w}$ for handlers labeled with \code{win}, and $\trans{c}{\neg \chfig(\chset, \chcard)}{l}$ for handlers labeled with \code{lose}. The locations $w$ and $l$ identify the partition of participants into winning and losing processes.
The variables $\chvar$ and $\winvar$ are irrelevant in this variant as we are only interested in the partition; therefore, they are omitted.
%While all participants again start in a location $c$, the winning participants move to a location $w$, while the losing participants take the transition to a location $l$.
%In valstore agreement, a process
%Here, all participants start in a $c$ location where their proposals are stored in their chvar, and the round ends with all participants moving to (the same) location $d$ with the winning value stored in their winvar.
%\valstore agreement, $w_i$ and $l_i$ are the same location $d_i$. 
%(denoted by the local transition $\trans{c_i}{\chfig(\chset, \chcard,
%  \chvar,\winvar)}{d_i}$),
%On the other hand, \wam agreement is denoted by two local transitions: a
%winning transition $\trans{c_i}{\chfig(\chset,
%  \chcard,\code{null},\code{null})}{w_i}$ and a losing transition
%$\trans{c_i}{\chfig(\chset, \chcard,\code{null},\code{null})}{l_i}$. Here, both
%$\chvar$ and $\winvar$ are irrelevant as we are only interested in partitioning
%the participants into winners (that move to $w_i$) and losers (that move to
%$l_i$). We denote the winning and losing transitions as
%$\trans{c_i}{\chfig(\chset, \chcard)}{w_i}$ and $\trans{c_i}{\neg
%  \chfig(\chset, \chcard)}{l_i}$, respectively, for convenience. 
%
%
%
%
%\input{localchfig}
%
\begin{figure}[t]
\vspace{-2em}
 \centering
\includegraphics[width=0.95\linewidth]{common/globalch.pdf}
\caption{Part of the global transition system depicting various \ch transitions.}
\label{fig:globalch}
\vspace{-1em}
\end{figure}

\closeparagraph{Example.} To illustrate the behavior of \ch transitions,
we focus on a 2-process system in a state $\gqs$ 
(the relevant parts of which are shown in \figref{globalch}). 

First, consider a scenario where the \valstore local transition
$\trans{c}{\chfig(\chset,1,pv,wv)}{d}$ is part of the process definition. The
state $\gqs$ is a valid \gcs state satisfying condition C1 since both processes
$P_1$ and $P_2$ are in location $c$ and have consistent participant sets (since $S_1 = S_2 = \{P_1,P_2\}$). 
Here, processes $P_1$ and $P_2$ propose the values $x$ and $y$, respectively, and try
to reach agreement on 1 value. The \ch transition $\trans{\gqs}{}{\gqe^{x}}$
(resp. $\trans{\gqs}{}{\gqe^{y}}$), shown in the top half of \figref{globalch}, models
\valstore \consagree where $x$ (resp. $y$) is the winning value stored in each
participant's $wv$ variable. Observe that both processes transition to the same
location $d$. 

Next, consider an alternate scenario where the \wam local transitions
$\trans{c}{\chfig(\chset,1)}{w}$, and $\trans{c}{\neg \chfig(\chset,1)}{l}$ are
part of the process definition. Again, $\gqs$ is a valid \gcs state.  Here,
processes $P_1$ and $P_2$ wish to pick one winner to transition to location $w$
while the loser transitions to location $l$.  The \ch transition
$\trans{\gqs}{}{\gqe^{P_1}}$ (resp. $\trans{\gqs}{}{\gqe^{P_2}}$), shown in the bottom half of 
\figref{globalch}, models \wam \consagree where $P_1$ (resp. $P_2$) is selected
as the winning process. Observe that the values of the proposal variable $pv$
and the agreement variable $wv$ are unchanged for both $P_1$ and $P_2$.\\


%\closeparagraph{Example.} \\
%To illustrate the behavior of \ch transitions, consider a 2-process system in the \llm where the \valstore local transition $\trans{c}{\chfig(\chset,1,pv,wv)}{d}$ as well as the \wam local transitions $\trans{c}{\chfig(\chset,1)}{w}$, and $\trans{c}{\neg \chfig(\chset,1)}{l}$ are part of the process definition. Further, assume that processes $P_1$ and $P_2$ have consistent participants sets (i.e., $\chset_1 = \chset_2 = \{P_1,P_2\}$).

%Then, the global state $\gqs$, shown in \figref{globalch}, is a valid \gcs state satisfying condition C1 since both processes $P_1$ and $P_2$ are in location $c$ and have consistent participant sets. The \ch transitions $\trans{\gqs}{}{\gqe^{x}}$ and $\trans{\gqs}{}{\gqe^{y}}$ (shown in \figref{globalch}) model \valstore \consagree where processes $P_1$ and $P_2$ propose the values $x$ and $y$, respectively, and try to reach agreement on one value. The global state $\gqe^{x}$ (resp. $\gqe^{y}$) encodes the scenario where \valstore \consagree concluded with $x$ (resp. $y$) as the chosen value written to the agreement variable $wv$. Observe that both processes transitioned to the same location $d$. On the other hand, the \ch transitions $\trans{\gqs}{}{\gqe^{w_1}}$ and $\trans{\gqs}{}{\gqe^{w_2}}$ (shown in \figref{globalch}) model \wam \consagree where processes $P_1$ and $P_2$ wish to pick one winner to transition to location $w$ while the loser transitions to location $l$. The global state $\gqe^{w_1}$ (resp. $\gqe^{w_2}$) encodes the scenario where \wam \consagree concluded with $P_1$ (resp. $P_2$) as the winning process. Observe that the values of the proposal variable $pv$ and the agreement variable $wv$ are unchanged.\\

%
%
%
%
%
%
%
%
%
We finally note that \valstore \consagree directly captures $k$-set
agreement~\cite{chaudhuri1990agreement} and can capture
Paxos~\cite{lamport1998part}\footnote{A \consprot protocol is required to
  satisfy three properties in the absence of faults: \emph{agreement} (all
  participants agree on the same value), \emph{validity} (the chosen value is
  among the proposed values), and \emph{termination}
  \cite{Lynch:1996:DA:525656}.  $\ch$ transitions satisfy agreement and
  validity by ensuring that the resulting $\winvar$ set is consistent across
  all participants and is a subset of the set of proposals.  Termination is
  guaranteed as $\chgt$ transitions are atomic.} by setting $\chcard$ to one.
Agreement protocols like Multi-Paxos~\cite{chandra2007paxos} and
Raft~\cite{ongaro2014search} can be modeled by using \wam agreement to elect a
leader, followed by the leader proposing values in subsequent rounds using \valstore
agreement.\\

%protocols as follows:
%\Wam \consagree can be used to model variants of Leader Election protocols as
%well as Multi-Paxos~\cite{chandra2007paxos} and Raft~\cite{ongaro2014search}:
%
%\begin{compactenum}[--]
%\item Leader Election: To elect $k$ leaders, use \wam agreement; create transitions $\trans{candidate}{\chfig(\chset, \chcard)}{leader}$ for the leader(s) to follow and $\trans{candidate}{\neg \chfig(\chset, \chcard)}{follower}$ for the rest.
%\item Multi-Paxos and Raft: To model such protocols, one can use \wam agreement to elect a leader, and have that leader propose values in subsequent rounds using \valstore agreement.
%\end{compactenum}
%\begin{compactenum}[--]
%\item Paxos: to agree on a single value, use \valstore agreement with $\chcard
%  =1$; create a transition $\trans{start}{\chfig(\chset,
%    \chcard,\chvar,\winvar)}{done}$ and interpret the value in $\winvar$ as the
%  chosen value.\footnote{A \consprot protocol is required to satisfy three
%    properties in the absence of faults: \emph{agreement} (all participants
%    agree on the same value), \emph{validity} (the chosen value is among the
%    proposed values), and \emph{termination} \cite{Lynch:1996:DA:525656}.
%    $\ch$ transitions satisfy agreement and validity by ensuring that the
%    resulting $\winvar$ set is consistent across all participants and is a
%    subset of the set of proposals.  Termination is guaranteed as $\chgt$
%    transitions are atomic.}
%\item $k$-Set Agreement: To agree on $k$ values, use \valstore agreement and interpret the values in $\winvar$ as the chosen $k$-set.
%\end{compactenum} 
%\editt{end}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%\closeparagraph{Example.} 
%\nour{do we need a \valstore example?}
%Consider a round of \wam agreement in a distributed system with 4 processes, $\chfig(\{1,2,4\}, 2)$ 
%where processes 1, 2, and 4 participate to choose two winners and process 3 is not interested.
%Thus, the set of proposals (omitting $\chvar$) is $\{1, 2, 4\}$ and 
%the set $\winset^*$ of all possible winner sets is 
%$\{ \{1, 2\},$ $ \{1,4\},$ $ \{2,4\} \}$.
%The behavior of the global transition system 
%in the \ch model, relevant to this agreement round, 
%is shown in~\figref{globalchoose}.
%The \ch transition abstracting this agreement round 
%originates in the \gcs state $c_1c_2x_3c_4$; here, 
%process 3 is in a {\em don't care} local state $x$.
%The \ch transition nondeterministically 
%ends in one of three possible \gce states, 
%each encoding one of the sets of winning proposals.\\
%Note that the \ch transition cannot originate in 
%the state $X_1C_2X_3C_4$ as it does not 
%satisfy the {\em Consistent Participants} precondition for this set of participants.\\
\para{Symmetry in the \ch Model}.  
In a global transition
system, $\M_{\ch} = (\GQ,q_0,\GT)$, in the \ch model, let $\GT_{\ch}$ denote
the set of all \ch transitions in the transition relation $\GT$.  Thus,
$\GT_{\ch}$ consists of transitions of the form $(\gqs, \gqe^\winset)$, where
$\gqs$ is a \gcs state and $\gqe^\winset$ is a corresponding \gce state.  Let
$\M = (\GQ,q_0,\GT\setminus \GT_{\ch})$ denote the global transition system
without the \ch transitions of $\M_{\ch}$.

\begin{lemma}
\label{lem:indexIndepOfCh}
If $\M$ is fully-symmetric, then $\M_{\ch}$ is fully-symmetric.
\end{lemma}
We refer the reader to \appref{chsymmetry} for the proof. 
Intuitively, the proof is based on the observation that 
\ch transitions are oblivious to the identities of the participants 
and are hence invariant under permutations over $\Ind$.\\

\noindent {\em Remark.} We do not make any symmetry-related assumptions about 
the specific agreement protocol implementation that the $\chgt$ transition 
encapsulates. Our abstraction is a safe overapproximation of possible
results of specific agreement implementations 
(including ones based on non-symmetric strategies such as ``process with maximum index wins'').

%\chris{Note that under this definition, the original \ch transition can be defined $\ch(\chset, \chcard) = \chfig(\chset, \chcard, self.pid)$, and $\bac$ can be defined $BaC(\chvar) = \chfig(\Ind, n, \chvar)$}.

























==> encoding-backup.tex <==
\section{Encoding \Counterexamples}
\label{sec:encoding}

%Our synthesis procedure (ref. \algoref{synthAlgo}) for solving \mpsp hinges on extracting counter-examples for when properties fail at any stage of the synthesis loop, and encoding such counter-examples as constraints to the oracle so that all interpretations exhibiting the same violation are ruled out. 
%In this section, we first define the nature of such counter-examples (but defer \emph{how} they are extracted to \secref{extraction}), then present an \emph{exact} encoding for such counter-examples. We will first focus on counter-examples to \emph{local properties} (i.e., \chwellbehavedness and \amenability) then handle counter-examples to \emph{global properties} (i.e., safety and liveness).

We now describe an \emph{exact} encoding of a counter example $\cex$ corresponding to a local or a global property violation to a constraint $\constraint$ that can be added to the \learner $\learnerSymbol$ to rule out that violation. The encoding is exact since the generated constraint $\constraint$ rules out exactly all interpretations $\interpretation \in \interpretations$ where the a candidate process %local or global semantics of 
$\pcomplete$ exhibits $\cex$ (as opposed to an over-approximation where $\constraint$ would rule out candidate processes that do not exhibit $\cex$, or an under-approximation where $\constraint$ would allow candidate processes that do exhibit $\cex$).\ourskip


%
%\subsection{Counter-Examples of Local Properties}
%Recall that a candidate \aml process $\pcomplete$ based on some process sketch $\psketch$ and interpretation $\interpretation$ has the local semantics $\isemantics = (\istates,\loq_0,\events,\itransitions, \idistransitions)$ where $\istates$ is the set of local states, $\loq_0$ is the initial state, $\events$ is the set of events and $\itransitions$ (resp. $\idistransitions$) is the set of enabled (resp. disabled) transitions under the current interpretation $\interpretation$. 
%Further, recall in the first two stages of the synthesis loop, we check if $\pcomplete$ satisfies \chwellbehavedness and \amenability conditions (i.e., $\isemantics \models \phaseCompSpec$ and $\isemantics \models \cutoffsSpec$).
%
%Naturally, a counter-example $\cex$ to \chwellbehavedness (resp. \amenability) is a ``subset'' of the local semantics $\isemantics$ such that $\cex \not \models \phaseCompSpec$ (resp. $\cex \not \models \cutoffsSpec$). We say that $\cex$ is a subset of $\isemantics$, denoted $\cex \subseteq \isemantics$, when it has a subset of its enabled and disabled transitions, i.e., $\cex = (\istates,\loq_0,\events,\itransitions' \subseteq \itransitions, \idistransitionsPrime \subseteq \idistransitions)$.

\subsection{Encoding \Counterexamples of Local Properties}
\label{sec:localEncoding}
%\item does not remove any interpretation without this substr
%\item does not miss any interpretation that has this substr
%\end{compactenum}

We start by defining the notion of \emph{concrete} local states, as it simplifies the presentation of the encoding. \ourskip %\editt{not happy about the placement of this, but can't find a better spot.}

\para{Concrete Local States.} We say a transition $t = \trans{\ls}{\action}{\ls'}$ based on action handler $\handler$ over action $\action$ is a \emph{sketch transition} if $\handler$ contains no uninterpreted functions in its guard or updates. A local state $\ls \in \istates$ is \emph{concrete} if (i) $\ls$ is the initial state $\ls_0$, or
(ii) there exists a sketch transition $\trans{\ls'}{}{\ls}$ where $\ls'$ is concrete. In other words, a local state $\ls$ is concrete if there exists a path from the initial state $\ls_0$ to $\ls$ in the process sketch semantics $\sksemantics$ and hence is always reachable regardless of the interpretation we obtain from the \learner.\ourskip

%existence
%realization
%materialization
%incarnation
%manifestation

%schema
%template
%fingerprint
%recipe
%condition

Since a \counterexample $\cex \subseteq \isemantics$ is effectively a set of enabled and disabled transitions, we show how we encode a single enabled/disabled transition, then lift the encoding to $\cex$. In what follows, let $\allConstraints$ be the set all well-typed constraints that the \learner $\learnerSymbol$ accepts. \ourskip

%\para{Manifestation Fingerprint 
\para{Encoding Enabled Local Transitions w.r.t. Interpretation $\mathbf{\interpretation}$.} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%C (universe of the local semantics):
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%t in T
%define C: trivial, skip.
%f1(s): ``the state s is reachable''
%f2(s,a): ``assuming the state s is reachable, s has action a''
%f3(s,a,s') ``assuming state s is reachable and s has action a, applying updates of action a on s yields s'''
%f4: a set S of states is reachable...
%[s]
%[s,a]
%[s,a,s']
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%A (universe of the oracle): 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%the atoms of the interpretation I
%define A: useful
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%B (interface we need to build): 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%manifestation fingerprint (formula) [[t]]
%define B: punchline first, then formalize.
%punch line:
%A \emph{manifestation fingerprint} 
An encoding of some enabled transition $t$ in $\cex$
is a formula 
$\fconstraint \in \allConstraints$ that
%over the atoms of the interpretation I that 
(i) is satisfied under interpretation $\interpretation$ (i.e., $\interpretation \models \fconstraint$) and (ii) implies that $t \in \itransitions$. Informally, such formula $\fconstraint$ acts like an interpolant between the logical encoding of the interpretation $\interpretation$ and the logical encoding of the transition $t$. In what follows, for some transition $t =  \trans{\ls}{\action}{\ls'}$ based on action handler $\handler$ over action $\action$, we show how to build the formula $\fconstraint$, denoted $\existsTr{\trans{\ls}{\act}{\ls'}}$ as a conjunction of the following predicates:\ourskip


%Given an interpretation $\interpretation$ and local semantics $\isemantics$ of completed process $\pcomplete$, a \emph{manifestation fingerprint} for some transition $t$ in $\isemantics$
%is a formula $\fconstraint \in \allConstraints$ that
%%over the atoms of the interpretation I that 
%(i) is satisfied under interpretation $\interpretation$ (i.e., $\interpretation \models \fconstraint$) and (ii) implies that $t \in \itransitions$. Informally, such fingerprint $\fconstraint$ acts like an interpolant between the logical encoding of the interpretation $\interpretation$ and the logical encoding of the transition $t$. In what follows, for some transition $t =  \trans{\ls}{\act}{\ls'}$, we show how to build the fingerprint $\fconstraint$, denoted $\existsTr{\trans{\ls}{\act}{\ls'}}$ as a conjunction of the following predicates:\ourskip
%elude to interpolants.
%A --> B --> C
%C (universe of the local semantics):
%TODO
%``partial eval''
%``good notation''



%A local state $\ls \in \istates$ is concrete if there exists a path from the initial state $\ls_0$ to $\ls$ in the \emph{program sketch} $\psketch$ \nour{can also define $\LS_{sk}$ and $\T_{sk}$ if need be.}. In other words, regardless of the interpretation we obtain from the oracle, $\ls$ is always reachable.\ourskip

\begin{compactenum}
\item the predicate $\reachable{\ls}$ indicating that the source state $\ls$ is reachable from the initial state $\ls_0$ under interpretation $\interpretation$. If $\ls$ is concrete, $\reachable{\ls}$ is simply $true$ (i.e., s is always reachable regardless of $\interpretation$). Otherwise, $\reachable{\ls}$ is defined as follows. Let $\mathcal{P}$ be the set of all paths from the initial state $\ls_0$ to state $\ls$. Then,
$$\reachable{\ls} \coloneqq \bigvee_{p\in \mathcal{P}} \existsTr{p}$$
where $\existsTr{p}$ for some path $p$ consisting of local transitions $t_1,\ldots,t_i$ is defined as $\existsTr{t_1} \wedge \ldots \wedge \existsTr{t_i}$.


\item 
the predicate $\hasAction{\ls}{\action}$ indicating that the process can perform action $\action$ from state $\ls$. The predicate $\hasAction{\ls}{\action}$ is defined as follows:
%. 
%Let $\guard(h')$ be the guard associated with handler $h'$. Let $h$ be the enabled handler over action $\action$ in state $\ls$ (i.e. $\valOf{\ls}{\guard(h)} = true$ under interpretation $\interpretation$).\footnote{There will only be one enabled handler over a given action in a particular state due to determinism assumptions.\nour{add: a?? a?? on the same state and similarly a!! and a!!, check picture}} Then, 
$$\hasAction{\ls}{\act} \coloneq (\guard(\handler)[\valOf{\ls}{\vars}/\vars] = true),$$
%
%$$\hasAction{\ls}{\act} \coloneq (\guard(\handler)[\valOf{\ls}{\vars}/\vars] = \valOf{\ls}{\guard(\handler)}),$$

%\editt{double check this\footnote{\nour{revise this to be: collect ufs, make it uf.partialEval(src) = uf.eval(src)}}}

where $\guard(\handler)[\valOf{\ls}{\vars}/\vars]$ is the guard $\guard(\handler)$ with each local variable $v \in \vars$ replaced by its value $\valOf{\ls}{v}$ in state $\ls$.



%\item 
%%\nour{account for different handlers}
%the predicate $\hasAction{\ls}{\act}$ indicating that an action $\act$ is available in state $\ls$. The predicate $\hasAction{\ls}{\act}$ is defined as follows. Let $\handlers(\act)$ be the set of handlers over action $\act$, and $\guard(h)$ be the guard associated with handler $h$. Then, 
%$$\hasAction{\ls}{\act} = \bigvee_{h \in \handlers(\act)} \guard(h)[\valOf{\ls}{\V}/\V],$$
%where $\guard(h)[\valOf{\ls}{\V}/\V]$ is the guard $\guard(h)$ with each variable $v \in \V$ replaced by its value $\valOf{\ls}{v}$ in state $\ls$.



%	\begin{compactenum}
%	\item If $\locname$ has no handler over the action $\act$, then  $\hasAction{\ls}{\act}$ is simply $false$ (i.e., the handler does not exist regardless of the current interpretation).
%	
%   	\item  
%   	If $\locname$ has a handler $h$ over $\act$ with handler predicate $pred(d_1,\ldots,d_i)$, then
%   	$$\hasAction{\ls}{\act} \coloneqq pred(\valOf{s}{d_1},\ldots,\sigmaOf{d_i}).$$
%   	\editt{(or .... )}
%   	$$\hasAction{\ls}{\act} \coloneqq pred(\ls(d_1),\ldots,\ls(d_i)).$$
%   	   	\editt{(or .... )}
%   	   	$$\hasAction{\ls}{\act} \coloneqq \ls(pred).$$
%   	   	   	
%Note that, if $pred(d_1,\ldots,d_i)$ contained no uninterpreted functions, then $\hasAction{\ls}{\act}$ evaluates to $true$ or $false$ irrespective of the current interpretation. Alternatively, if it contained uninterpreted functions, then we are left with a boolean formula over functions in $\uFuns$ with domains drawn from $\sigma$.
%    
%	\end{compactenum}

%	\nour {Keeping this for now but it needs polishing.}

{\em Example.} Let $\uf(a,b)$ be an uninterpreted function over local \code{int} variables $a$ and $b$. Let the local state $\ls \coloneqq \{\locVar = \code{Z}, a=1,b=2\}$, and let the local guard of action handler $\handler$ over action $\action$ in location \code{Z} be 
$\guard \coloneqq \uf(a,b) > 7 \vee a=2$. Then $\hasAction{\ls}{\action}$ = \big((
$\uf(\valOf{\ls}{a},\valOf{\ls}{b}) > 7 \vee
\valOf{\ls}{a}=2)  = true)\big)$ 
which is 
$\big((\uf(1,2) > 7 \vee
1=2) = true\big)$ which simplifies to $\uf(1,2) > 7$.


%\editt{simplified the example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\em Example.} Let $\uf_1(a,b,c)$ and $\uf_2(a,b)$ be uninterpreted functions over local \code{int} variables $a$, $b$ and $c$. Let $\ls \coloneqq \{\locVar = \code{Z}, a=1,b=2,c=3\}$, and let the local guard of action handler $h$ over action $\action$ in location \code{Z} be 
%$\guard \coloneqq \uf_1(a,b,c) \wedge (\uf_2(a,b) > 7 \vee a=2)$. Then $\hasAction{\ls}{\action}$ = (
%$\uf_1(\valOf{\ls}{a},\valOf{\ls}{b},\valOf{\ls}{c}) \wedge
%(\uf_2(\valOf{\ls}{a},\valOf{\ls}{b})  > 7 \vee
%\valOf{\ls}{a}=2)  = true)$ 
%which is 
%$(\uf_1(1,2,3) \wedge 
%(\uf_2(1,2) > 7 \vee
%1=2) = true)$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%$\guard \coloneqq \code{\uf}_1\code{(a,b,c) \&\& (}\uf_2\code{(a,b) > 7 || a==2)}$. Then $\hasAction{\ls}{\act}$ is defined as follows: 
%$\code{\uf}_1\code{(\valOf{\ls}{a},\valOf{\ls}{b},\valOf{\ls}{c}) \&\& (}\uf_2\code{(\valOf{\ls}{a},\valOf{\ls}{b})  > 7|| \valOf{\ls}{a}==2)} $ 
%which is $ \code{\uf}_1\code{(1,2,3) \&\& (}\uf_2\code{(1,2) > 7|| 1==2)}$.

\item the predicate $\goesTo{\ls}{\action}{\ls'}$ indicating that $\ls$ goes to $\ls'$ on action $\action$.	The predicate $\goesTo{\ls}{\action}{\ls'}$ is defined as follows. 
Let $\update(\handler)$ denote the set of updates of the form $\lhs \coloneq \rhs$ of handler $\handler$ over action $\act$. Then,	
	$$\goesTo{\ls}{\action}{\ls'} \coloneqq \bigwedge_{\lhs \coloneq \rhs \in \update(\handler)} \ls'(\lhs) = \rhs[\ls(\vars)/\vars].$$
%	\footnote{We treat \terma{goto} statements as an assignment to a special ``location'' variable.} 	
{\em Example.} Let the set of updates have the single update $a \coloneqq \uf(b,c)$ and $\ls,\ls'$ be $\{\locVar = \code{Z}, a=1,b=2,c=3\}$ and $\{\locVar = \code{W},a=5,b=2,c=3\}$.
Then $\goesTo{\ls}{\action}{\ls'}$ is:
$\valOf{\ls'}{a} = \uf(\valOf{\ls}{b},\valOf{\ls}{c})$ which is 
$\uf(2,3)=5.$ \ourskip
\end{compactenum}


Putting it all together, we have:
$$
%\fconstraint = 
\existsTr{\trans{\ls}{\action}{\ls'}} = 
\reachable{\ls} \wedge 
\hasAction{\ls}{\action} \wedge 
\goesTo{\ls}{\action}{\ls'}$$


The intuition behind breaking the encoding of each local transition to the three components above is that some of the \chwellbehavedness conditions %in \cite{quicksilver} 
leave parts of a transition unspecified. For instance, the predicate ``the local state $\ls$ can react to event $\event$'' corresponds to a local transition $\trans{\ls}{\acting{\event}}{*} \in \itransitions$ with encoding $\reachable{\ls} \wedge \hasAction{\ls}{\action}$.
\ourskip

%\para{Manifestation Fingerprint of 
\para{Encoding Disabled Local Transitions w.r.t. Interpretation $\mathbf{\interpretation}$.}
An encoding of some disabled transition $t = \trans{\ls}{\action}{\bot}$ in $\cex$
is a formula $\fconstraint \in \allConstraints$ defined as $ \existsTr{t} = \reachable{\ls} \wedge \hasNoAction{\ls}{\action}$ where $\reachable{\ls}$ is defined as before and $\hasNoAction{\ls}{\action}$
is a predicate indicating that the process cannot perform action $\action$ from state $\ls$. Let $t$ be based on action handler $\handler$ over action $\action$. Then, the predicate $\hasNoAction{\ls}{\action}$ is defined as follows:
$$\hasNoAction{\ls}{\action} \coloneq (\guard(\handler)[\valOf{\ls}{\vars}/\vars] = false),$$
%\editt{double check this\footnote{\nour{revise this to be: collect ufs, make it uf.partialEval(src) = uf.eval(src)}}}
where $\guard(\handler)[\valOf{\ls}{\vars}/\vars]$ is the guard $\guard(\handler)$ with each local variable $v \in \vars$ replaced by its value $\valOf{\ls}{v}$ in state $\ls$.\ourskip










\para{Encoding a Local \Counterexample $\cex$ w.r.t. Interpretation $\mathbf{\interpretation}$.}
Finally, an encoding for some $\cex = (\istates, \loq_0, \events, \itransitions, \idistransitions)$, is a formula $\fconstraint \in \allConstraints$, denoted $\existsTr{\cex}$, defined as expected:
$$
\fconstraint =  \existsTr{\cex} = 
\bigwedge_{t \in \{\itransitions \cup \idistransitions\}} \existsTr{t}
$$
%$$
%\fconstraint =  \existsTr{\cex} = 
%\bigwedge_{t \in \itransitions} \existsTr{t}
%\wedge 
%\bigwedge_{t \in \idistransitions} \existsTr{t}.
%$$
\para{From \Counterexample Encoding $\mathbf{\fconstraint}$ to a Constraint $\constraint$.} In order to rule out any interpretation $\interpretation \in \interpretations$ that exhibits $\cex$, we add the constraint $\constraint = \neg \fconstraint$ to the \learner $\learnerSymbol$.
%







%
%
%
%\subsection{Counter-Examples of Global Properties}
%Recall that $\pcomplete$ has the global semantics $\iglobalSemantics = (\iGQ,\gq_0,\events,\iGT, \iDisGT)$, where $\iGQ$ is the set of global states, $\gq_0$ is the initial global state, 
%$\events$ is the set of events,
%and  $\iGT$ is the set of global transitions.
%Further, recall that in the last two stages of the synthesis loop, we check if cutoff-sized system based on $\pcomplete$ is safe and live (i.e., $\isemantics \models \safetySpecc$ and $\isemantics \models \livenessSpec$). 
%
%
%Similar to counter-examples of local properties, a counter-example $\cex$ to safety (resp. liveness) is a ``subset'' of the global semantics $\iglobalSemantics$ such that $\cex \not \models \safetySpecc$ (resp. $\cex \not \models \livenessSpec$). We say that $\cex$ is a subset of $\iglobalSemantics$, denoted $\cex \subseteq \iglobalSemantics$, when it has a subset of its enabled and disabled global transitions, i.e., $\cex = (\iGQ,\gq_0,\events,\iGT' \subseteq \iGT,\iDisGTPrime \subseteq \iDisGT)$.
%
%
%
%



\subsection{Encoding \Counterexamples of Global Properties}


As before, we will focus on the encoding of a global transition, then lift that to the encoding of a \counterexample $\cex \subseteq \iglobalSemantics$.\ourskip

\para{Encoding Global Transitions w.r.t. Interpretation $\mathbf{\interpretation}$.}
For some global transition $r = \trans{\gq}{\event}{\gq'}$, we denote by $\activeTrs(r)$ the local transitions that processes in $\gq$ locally use to end in $\gq'$. That is, $\activeTrs(r) = \{t \in \itransitions \mid \exists \p_{\interpretation,i} : t = \trans{\gq[i]}{\acting{\event}}{\gq'[i]} \vee t = \trans{\gq[i]}{\reacting{\event}}{\gq'[i]}\}$ %\editt{there must be a better way of doing this..}. 
We then define the encoding $\existsTr{r}$  as a constraint $\fconstraint \in \allConstraints$ as:
$$
\existsTr{r} = \bigwedge_{t \in \activeTrs(r)}{\existsTr{t}}.
$$

Note that the predicates $\reachable{\gq}$, $\hasAction{\gq}{\event}$, $\goesTo{\gq}{\event}{\gq'}$, and $\hasNoAction{\gq}{\event}$ as well as the encoding for the global disabled transitions can be defined 
similar to their local counterparts from \secref{localEncoding}.
\ourskip

\para{Encoding a Global \Counterexample $\cex$ w.r.t. Interpretation $\mathbf{\interpretation}$.}
An encoding for some $\cex = (\iGQ,\gq_0,\events, \iGT,\iDisGT)$, is a formula $\fconstraint \in \allConstraints$, denoted $\existsTr{\cex}$, defined as:
$$
\fconstraint =  \existsTr{\cex} = 
\bigwedge_{r \in \{\iGT \cup \iDisGT\}} \existsTr{r}
$$

As before, in order to rule out any interpretation $\interpretation \in \interpretations$ that exhibits $\cex$, we add the constraint $\constraint = \neg \fconstraint$ to the \learner $\learnerSymbol$.
%%
%\para{From Counter-Example Encoding $\mathbf{\fconstraint}$ to a Constraint $\constraint$.} In order to rule out any interpretation $\interpretation \in \interpretations$ that exhibits the $\cex$, we add the constraint $\constraint = \neg \fconstraint$ to the oracle $\oracle$.
%%

%\edit{random and probably no longer needed}
%
%If the destination state is unspecified, (i.e., $\trans{\ls}{\action}{*}$), then the above predicate becomes:
%$$\existsTr{\trans{\ls}{\action}{*}} = \reachable{\ls} \wedge \hasAction{\ls}{\action} $$
%
%
%Finally, for some set $S' \subseteq \istates$ of states, we define $\reachable{S'}$ as:
%
%$$\reachable{S'} \coloneqq \bigwedge_{s \in S'} \reachable{s}$$
%
%
%
%Let us assume the following finite error trace to some error state:
%
%$$
% \tau = q_0 \xrightarrow{(e_1,M_1,v_1)}  q_1 \xrightarrow{(e_1,M_1,v_1)}  \ldots  \xrightarrow{(e_m,M_m,v_m)}  q_{err} 
%$$
%
%Then, the encoding of the trace $\tau$ is essentially
%
%$$
%\llbracket \tau \rrbracket = \bigwedge_{q \xrightarrow{e} q' \ \in \ transitions(\tau)} \big(\llbracket e\mid q \rrbracket \wedge \llbracket q' \mid q, \ e\rrbracket  \big)
%$$
%
%Note that we do not really care about the source here because the initial state is always concrete and every other state is basically reachable by being on the path.
%




==> evalfigs.tex <==
\section{Evaluation}
\input{chubby-dsl}
\input{sdr-dsl}
\input{DMRfig-dsl}	
\input{sats-dsl-full}
\input{kvs-dsl}


\subsection{Benchmarks}
\label{app:evalfigs}
In this section, we provide specifications and \aml description for our benchmarks from \secref{evaluation}. \kinarach can successfully verify all of our case studies.\\
%The transition diagrams demonstrate the {\em complete} implementation, with the holes we synthesize marked in dashed red boxes. \\
%\noindent{\em Remark.} In this work, we focus on parameterized verification for safety properties. However, in order to enable synthesis, we also support checking if a system is \emph{live} for the cutoff number of processes.  The expected live behavior of (executions of) the global
%transition system $\M$ is specified by augmenting $\M$ with accepting states $A \subseteq \GQ$ to capture violations liveness 
%specifications. An infinite execution of $\M$ is {\em accepting} if it visits accepting states in $A$ infinitely often. The system $\M$ is live if it has no accepting infinite execution. 

\para{Chubby Application}\\
%\input{common/chubbyfig}
\noindent{\em Protocol description.} We evaluate a distributed lock service with a leader node, which has the following behavior. All processes begin as candidates to be chosen as the leader. Upon performing a \PartitionCons operation, one node is selected as the leader, while others are designated as replicas. The leader fields requests from the environment and forwards them to the replicas. Once timeout signal is received, the leader broadcasts to the system that it is stepping down, and all processes become candidate leaders again.\\
\noindent{\em Specifications.} The safety properties for this system is that %: (1)
there is at most one leader at a time.\\

%; and (2) each write is committed to all
%replicas before it is acknowledged. \chris{is this second safety property still being checked?}
%The liveness properties
%are: (1) client reads and writes must eventually be acknowledged; and (2) on a
%timeout, all servers must go back to the $Candidate$ state where a new server
%is elected. 
%\closeparagraph{Synthesis Completions.}
%%Since there are no guards and updates for Chubby,
%%the completion here had a different style: for the actions in the dashed red
%%boxes (\figref{chubby}), the \emph{next state} is left unspecified. The job of the synthesis to
%For the actions in the dashed red
%boxes (\figref{chubby}), the \emph{next state} is left unspecified. The job of the synthesis to answer questions like: in the case of a timeout, where should the leader
%transition to, and how should the replicas react? Also, how should the leader
%server react to a read or write? How should the replicas react to a write?. In
%addition to that, we also allow the synthesis procedure here to figure out the
%right number of winners for \consagree.
%The cutoff is 2 according to \lemref{cutofflemma}.

\para{Distributed Smoke Detector}\\
%\input{common/introfig}
\noindent{\em Protocol description.} We consider a distributed smoke detector whose behavior is as follows. Upon detecting smoke, the
detectors coordinate using an \consagree protocol to choose at most two processes
to contact the fire department.\\ %This example displays the utility of allowing the set of participating processes in the \consagree operation to be dynamically constructed: only detectors that detected the smoke coordinate as opposed to all the detectors in the system.
\noindent{\em Specifications.} 
The safety properties for the Distributed Smoke Detector system, depicted in~\figref{sdrcode}, are: (1) at most two detectors can contact the fire department; and (2)
detectors that did not detect fire will never report detecting one.
%The liveness property is: if a fire was detected, then the system should eventually contact the fire department. 
With a reset signal, the verifier must make sure the specifications are met for each
\emph{round} of the system: before the detectors go back to the detecting a
new fire, they must correctly handle the current one.\\


%\closeparagraph{Completions.} We omitted the guards and updates in the dashed red
%boxes and were able to synthesize the correct completions to satisfy the
%specification. The omitted parts correspond to interesting questions the
%developer of such system might have. For example, should the detector attempt
%to build a participant set of detectors that sensed a fire? what should a
%detector do upon receiving a message from another detector? After the message
%exchange is done, should the detector attempt to contact the fire department
%or is other processes going to do so?.
%Since all detectors go back to the initial state at the same time, this system is around-based and the cutoff is 3 according to \lemref{cutofflemma}.


\begin{figure*}[ht]
\centering
%\fbox{
% trim={<left> <lower> <right> <upper>}
\includegraphics[width=0.4\linewidth,clip, trim=2.5cm 0cm 2cm 0.3cm]{varyN-total-time-log.pdf}
%}
\caption{Run time w.r.t. the number of processes.} 
\label{fig:varyN}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}{0.4\linewidth}
%\fbox{
% trim={<left> <lower> <right> <upper>}
\includegraphics[width=\linewidth,clip, trim=2.3cm 0cm 2cm 0cm]{varyK-check-time.pdf}
%}
\caption{Check Time.} 
\label{fig:varykchecktime}
\end{subfigure}
\begin{subfigure}{0.4\linewidth}
%\fbox{
% trim={<left> <lower> <right> <upper>}
\includegraphics[width=\linewidth,clip, trim=2.3cm 0cm 2cm 0cm]{varyK-solve-time-log.pdf}
%}
\caption{Verification Time.} 
\label{fig:varyksolvetime}
\end{subfigure}
\caption{Run time as a function of partition cardinality.} 
\label{fig:varyK}
\end{figure*}

\para{Distributed Mobile Robotics(DMRs)}\\
\noindent{\em Protocol description.} As a larger case study, we model the system presented in~\cite{Desai.DRONAFrameworkSafe.X.2017} where a set of robots share a workspace with obstacles, and need to coordinate their movements. The robots coordinate to create a motion plan by successively choosing each robot to create a plan while taking into account the previous robots' plans. %We model this system in our \ch model: 
The robots choose one robot to make a plan, then the remaining robots re-enter \consagree to choose a second robot and so on. 
As in SATS, each round of \consagree determines the participant set of the next, but unlike SATS, the number of \consagree rounds is not statically bounded.\\
\noindent{\em Specifications.} The safety property here is that exactly one robot can be planning at a given time, hence no collision will happen. We abstract away from the mechanics of creating the plan itself.\\
%The liveness properties enforce that any submitted task should eventually be executed.

%\closeparagraph{Completions.} As shown in \figref{DMRfig}, the holes are similar to those of the smoke detector. Additionally, a hole corresponding to how should the robot handle a message from another robot that is done planning.
%The cutoff for this example is 3, according to ~\lemref{cutofflemma}.%\footnote{With some relaxation of the free path requirement: we allow broadcast-receive transitions that lead to a state with a free path.}.

%.\nour{double check lemma ref}

%\milind{Should this be in the main paper?} Note that DMR's operational model, unlike our other examples, does not satisfy the constraints required to guarantee cutoff---synthesis cannot guarantee that cutoffs will not change due to an inapt completion. Nevertheless, we manually ascertain that the synthesized protocol's cutoff is the same in both the high-level model and the operational model.



%\swap{
%%origial: sats, kvs
%\para{Consortium.} Consortium is a distributed system where a set of actors want to reach a decision based on information they gather individually. In order to do this efficiently, a subset of the actors are elected and trusted with making a decision that is then announced to the rest of the actors. This resembles scenarios where a trade off between trust and performance is needed (e.g., a consortium blockchain~\cite{libraref,hyperledgerref}).  As shown in \figref{consortiumcode}, an actor starts in the \code{Election} location and coordinates with all other actors (\lineref{elect}) to pick at most two actors to move to the \code{Deliberate} location where the actors are trusted to make a decision for everyone. The remaining actors move to the \code{Wait} location where they  expect to be informed once the elected actors agree on a decision. The elected actors in \code{Deliberate} may be influenced (by the environment) to update their proposal. From there, the elected actors may initiate agreement (\lineref{vc}) over the proposed values, moving to \code{Decided} location where they choose one of them (\lineref{share}) to announce the agreed-upon value to the rest of the actors (Lines \ref{line:wins}, \ref{line:wine}). All actors then go back to the initial location to start further rounds. The safety property for this system is that all actors eventually agree on the decided value. 
%\input{consortium-dsl}
%\para{Small Aircraft Transportation System (SATS).} The \aml process definition for the SATS system is shown in ~\figref{satscodefull}
%\input{sats-dsl-full}
%}
%{
%replacement: consordium
\para{Small Aircraft Transportation System (SATS).}\\
The goal of NASA's SATS protocol~\cite{satsref}
is to increase access to small airports without control towers by allowing aircraft
to coordinate with each other to operate safely upon entering the airport airspace.
For the {\em landing} part of the protocol, the aircraft coordinate to choose successive subsets of
aircraft to progress to the next phase of landing, until just one aircraft is chosen
to land at a time; thus, the protocol relies on multiple rounds of distributed
agreement, in particular, (multi-)leader election.\\
In \figref{satscodefull}, we present the process definition for the
SATS landing protocol in \aml. An aircraft starts in a
\texttt{Fly} location and coordinates with other aircraft (\lineref{pc1}) to pick at most four
aircraft to move to the \texttt{Enter} location where the aircraft enter the
airport airspace; only four aircraft are allowed in the airport airspace
at a time to ensure there is enough room for any aircraft that misses its final
approach. Upon entering the aircraft airspace, the aircraft coordinate (\lineref{pc2}) to pick
at most two aircraft to move to a left holding location, \texttt{HoldLeft} 
and at most two aircraft to move to a right holding location, \texttt{HoldRight}; 
each holding location accommodates at most two aircraft by having 
each aircraft circle at a different altitude while waiting. The aircraft continue to coordinate until a single aircraft can descend to its final approach and land.\\
The safety properties for the SATS landing protocol, provided by NASA, include: (1) there are a total of at most four aircraft across the airport vicinity, and 
(2) there at most two aircraft across the locations 
\termb{HoldLeft}, \termb{HoldRight}.
\para{Distributed Key-Value Store.} Consider 
a distributed key-value store consisting of a group of replicated processes with data. %\roopsha{with data?}.
The desired functionality is to present
a consistent data model to clients who may access the data from an
arbitrary replica. One strategy is to perform consensus among
the replicated processes whenever any of them receives a request to change
the stored data. 

In \figref{kvscode}, we model a simple key-value store in the spirit of Redis~\cite{radisref} in \aml. For ease of presentation, we skip key indexing logic
and present a single-key system. The system begins with all
processes in an \code{Idle} location. 
If a process
receives a \code{get} request (\lineref{kvsget}) while in this location, it transitions to the \termb{Ret} location where it responds with its stored value.
Upon receiving a \code{put} request (\lineref{kvsput}) with some value,
a process must determine its effect on the collective data model. 
If the value 
is the same as the current stored value, no change is required and the process stays in \termb{Idle}. If the value differs from the stored value, the process moves
to the \termb{Agree} location to perform consensus with the other processes; 
since multiple processes may have received a \termb{put} message, 
they all must agree on a single value to store.
The safety property for this system is that no two processes in \code{Ret}
have different values in their \code{stored} variables, ensuring the clients have a consistent view of the data. 
%}


%%\subsection{Distributed Key-Value Store}
%%\input{common/KVStorefig}
%%\closeparagraph{Specifications.} The safety property/ies of this system, is that any two processes in the Idle state must have the same stored value, so any read request from the environment will be serviced with the same value, regardless of which process receives the request.% The liveness properties enforce that any submitted task should eventually be executed.
%%
%%\closeparagraph{Completions.} The goal here is to check if the processes need to involove \consagree upon a write request or if the value stored is unchanged.
%As shown in \figref{DMRfig}, the holes are similar to those of the smoke detector. Additionally, a hole corresponding to how should the robot handle a message from another robot that is done planning. The cutoff for this example is 3, according to ~\lemref{newcutoffLemma}.



%\chris{We had a problem in the value store benchmark with the internal transition from Idle to Decide, because this meant that every state in all the same guards as Idle (i.e. Idle and Agree) is required to have a transition to a state in all the same guards as Decide (everything except Idle and Agree). Since there are no internal transitions from Agree, and we must leave it, we have a problem. We solve this problem by reasoning that the multi-sender broadcast (value-store consensus) can always eventually happen. We know it can always happen, because every state outside of \{Idle, Agree\} can reach \{Idle, Agree\} via internal transitions (they are in the same phase per the phase analysis), so it is always possible to move all processes into \{Idle, Agree\} perform consensus, and then move the processes back to where they were via internal transitions. This preserves compatibility with respect to checking reachability.}


%\subsection{Small Aircraft Transportation System (SATS)}

%\closeparagraph{Protocol Description.}
%As shown in~\figref{sats}, an aircraft starts in \st{Fly} state. The
%aircraft then approaches the airport and head to a holding zone that can be either on the
%\emph{left} or the \emph{right}, represented by \st{HoldLeft} and \st{HoldRight}, respectively. Each holding zone can accommodate two aircraft. From either the left or the right, an aircraft
%may try to approach a \st{Base} where it attempts to approach the runway and
%land. In that \st{Base} zone, only one aircraft may move to the \st{Final
%Approach} zone where it can safely attempt to land, entering the \st{Landed} state. However, due to unforeseen
%reasons (e.g. ice on the runway), the pilot may decide to abort landing. At
%that point, the aircraft needs to head to a miss zone either on the left or the
%right, \st{MissLeft} and \st{MissRight}, respectively. From there, the aircraft goes back to the assigned holding zone and
%attempts the landing again.
%
%%\input{satsfig}
%%\nour{use whatever convention we use in figures here:}
%This is an instance where it is useful to allow the \ch transitions to also
%return the winner and loser sets to the participants. For example, $set_2$ is
%the winning set of \chfig$(set_1,4)$ and $set_3$ and $set_4$ are the winning and
%losing sets of \chfig$(set_2,2)$, respectively. Building $set_5$ requires the
%processes to communicate as in the smoke detector examples, we omit the
%communication states to keep the presentation simpler.
%Note that Table~\ref{table:results} includes the four states necessary to build $set_5$, but not shown here, in its characterization of SATS.

%\closeparagraph{Specifications} 
%The safety properties were started in \secref{intro}.
%, given by NASA, are as follows:
%\begin{itemize}
%\item While any number of aircraft can be in the \st{Fly} and \st{Landed} states, no more than four aircraft total can be in any of the other states.
%%\item No more than two aircraft can be on any side.\milind{This specification isn't very precise -- how is it different than the ones about hold left, hold right, miss left, and miss right below?}
%\item Only one aircraft is allowed on the \st{FinalApproach} state.
%\item No more than two aircraft allowed in \st{HoldLeft} (\st{HoldRight})
%state.
%\item No more than two aircraft allowed in \st{MissLeft} (\st{MissRight}) state.
%\item At most two aircraft are assigned to miss left (right) at any time.
%\end{itemize}
%For liveness, the protocol description states that all aircraft
%land in order of sequence number. However, enforcing this property breaks symmetry. Instead, we relax this property to ``an airplane entering the airport will land'', and leave enforcing sequential ordering to the non-deterministic results of consensus, outside of our verification scope.

%  However, since we are under
% the symmetric settings and any ``order'' of the processes would render
% symmetry unusable, we relax this to require that eventually, an aircraft will
% land. Enforcing sequence numbers boils down to instantiating a particular
% strategy for how \ch should pick its winners. Our \ch implementation is
% general and handles all the possible landing sequences.

%\closeparagraph{Completions}. The completions in this system corresponded to the right cardinalities of the \consagree operations needed to meet the specifications. Additionally we synthesize the 
%actions of the pilot attempting to land. In particular, which direction should
%the pilot take in case of an abnormal condition. The cutoff value for this example, is 5, according to \lemref{cutofflemma}. %\nour{double check lemma ref}
%The variant of SATS we consider, uses a more-complicated communication mechanism (like that of the Smoke Detector example) to build $BaseSet$.
%\input{common/satsfig}


%\input{introfig_onerep}

%\newpage

\subsection{Additional Experiments}
\label{app:evalextra}
We examine the effect of varying the number of processes, the cardinality of the agreement primitives, and the variable domains on the run time of \kinarach. The run time grows exponentially with the number of processes, as shown in~\figref{varyN}. All experiments time out beyond 10 processes given a 30-minute limit. This highlights the importance of small cutoffs to enable practical parameterized verification.

As shown in \figref{varykchecktime}, when varying the partition cardinality for the benchmarks that use \PartitionCons, the time needed to check the \chwellbehavedness and \amenability conditions is not affected, as such checks are performed on the local process semantics. Naturally, varying the cardinality causes the cutoff values to increase, so the verification time taken to verify the correctness of the cutoff-sized systems grows exponentially, as depicted in \figref{varyksolvetime}. 

For benchmarks that use \ValueCons, increasing the value domain size beyond the minimum needed by their specification causes exponential blowup in \kinarach. Addressing this bottleneck is a key target for future work.



==> extraction-backup.tex <==
\section{\Counterexample Extraction}
\label{sec:extraction}
%In the previous section, we presented a uniform, exact encoding for counter-examples corresponding to failures of local and global properties. In this section, we present the properties themselves, and how counter-examples are extracted during the synthesis procedure.

%In the previous section, we presented a uniform, exact encoding for counter-examples corresponding to failures of local and global properties. In this section, we present the properties themselves, and how counter-examples are extracted during the synthesis procedure.
%




Our synthesis procedure (ref. \algoref{synthAlgo}) for solving \mpsp hinges on extracting \counterexamples for when properties fail at any stage of the synthesis loop, and encoding such \counterexamples as constraints to the \learner so that all interpretations exhibiting the same violation are ruled out. 
In this section, we present the various properties a correct process $\pcomplete$ must meet as well as their corresponding \counterexamples. For the reminder of this paper, we will refer to \chwellbehavedness and \amenability conditions as \emph{local properties} and safety and liveness specifications as \emph{global properties}.


\subsection{Local Properties}
\Chwellbehavedness and \amenability conditions ($\phaseCompSpec$ and $\cutoffsSpec$, respectively) are introduced in \cite{Jaber.QuickSilver.OOSLA.2021} as sufficient conditions over the local semantics of some \aml process $\p$ and permissible safety specifications $\safetySpec$ that render the parameterized verification problem efficiently decidable.
%In general, such 
These conditions are specified as first-order logic formulas over the local semantics of a \aml process. The exact set of conditions are detailed in \appref{extractionApp}. %\nour{or \cite{quicksilver}?}.

\subsection{\Counterexamples of Local Properties}
Recall that a candidate \aml process $\pcomplete$ based on some process sketch $\psketch$ and interpretation $\interpretation$ has the local semantics $\isemantics = (\istates,\loq_0,\events,\itransitions, \idistransitions)$ where $\istates$ is the set of local states, $\loq_0$ is the initial state, $\events$ is the set of events and $\itransitions$ (resp. $\idistransitions$) is the set of enabled (resp. disabled) transitions under the current interpretation $\interpretation$. 
Further, recall in the first two stages of the synthesis loop, we check if $\pcomplete$ satisfies \chwellbehavedness and \amenability conditions (i.e., $\isemantics \models \phaseCompSpec$ and $\isemantics \models \cutoffsSpec$).

Naturally, a \counterexample $\cex$ to \chwellbehavedness (resp. \amenability) is a ``subset'' of the local semantics $\isemantics$ such that $\cex \not \models \phaseCompSpec$ (resp. $\cex \not \models \cutoffsSpec$). We say that $\cex$ is a subset of $\isemantics$, denoted $\cex \subseteq \isemantics$, when it has a subset of its enabled and disabled transitions, i.e., $\cex = (\istates,\loq_0,\events,\itransitions' \subseteq \itransitions, \idistransitionsPrime \subseteq \idistransitions)$.

\subsection{Extracting \Counterexamples to Local Properties}
We now discuss how one can extract a \counterexample $\cex$ of some local property, say, $\prop$.
%
%\edit{give the general procedure of doing it}
%
%**Counter Examples to Local Correctness Properties ($cex$)**
%Now, since the properties are over the local semantics $\semantics$, 
Given a candidate \aml process $\pcomplete$, when \tool concludes that a property $\prop$ fails (i.e., $\isemantics \not \models \prop$), then we need to extract a \counterexample $\cex \subseteq \isemantics$ such that $\cex \not \models \prop$ or equivalently, $\cex \models \neg \prop$.
%Is cex a small model property?
In other words, $\cex$ is an \emph{explanation} for why the property failed.
%“If the verification failed, why did it fail? which parts of the local semantics made it fail?”
The extraction procedure for a \counterexample $\cex$ proceeds as follows:
%The current procedure followed (manually) so far
\begin{compactenum}

\item Consider an arbitrary local property $\prop$.
\item Consider the negation of that property, $\neg \prop$, in disjunctive normal form (DNF) $\neg \prop = \cube_1 \vee \cube_2 \vee \ldots$ where each cube $\cube_i = \literal_1 \wedge \literal_2 \wedge \ldots$ is a conjunction of literals.% or their negations.
%$(x_1 \wedge x_2 \wedge \ldots ) \vee (x_3 \wedge \neg x_4 \wedge \ldots ) \vee \ldots$
\item For each of literal $\literal$ , the user must provide a procedure to extract a (minimal) subset $\literalWitness$ of the local semantics such that  $\literalWitness \models \literal$.
\item A counter example $\cex$ is the union of the witnesses $\literalWitness_1 , \literalWitness_2 , \ldots$ of all literals of some cube $\cube$ of $\neg \prop$. 
Since $\cex \models \cube $ and $\cube \Rightarrow \neg \prop$, we know that $\cex \models \neg \prop$ (or equivalently, $\cex \not \models \prop$).
\end{compactenum} 



In this work, we studied the \chwellbehavedness and \amenability conditions, obtained all the literals in the negations of such conditions, and equipped \tool with the needed \counterexample extraction procedures for these literals. We refer the interested reader to \appref{extractionApp} for details. Finally, we emphasize that the system designer does not need to provide any extraction procedures to use \tool.

%We refer the interested reader to \appref{localExtraction} for the list of \chwellbehavedness and \amenability conditions, the literals that appear in their negation, as well as the extraction procedures for these literals. 


\input{sec5example}


%\begin{verbatim}
%example for sec 6:
%1 -> 1
%2 -> Leader
%3 -> Replica
%4 -> [1,3] = true, [1,4] = false
%5 -> Candidate
%6 -> Return
%
%problem 
%1. state Leader13 --> Candidate13 goes to a state where it can lose election [Candidate --> ... --> Leader13 --> Candidate13] (1,2,4,5)
%3. Cand13 can react to elect:l (true)
%4. the action is firable, because Cand13 can fire it [Cand13 --w:elect --> *](true)
%5. samePhase (Leader13, Return14) [dest of elect: leader11 is dest state to elect + leader11-->leader13 + leader11-->leader14 --> Return14] (1,2,4,6)
%6. Return14 does not have access to l:elect [concrete](true)
%
%1,2,4[1,3] = true,4[1,4] = false,5,6
%\end{verbatim}}

%\edit{ref some examples in the appendix for both phase comp and amenability}



\subsection{Global Properties}
If a candidate \aml process $\pcomplete$ meets its \chwellbehavedness and \amenability conditions, then it belongs to the \effdecidable fragment of \aml, and a cutoff $c$ exists. It then remains to check if the system $\iglobalSemantics(c)$ is safe and live (i.e., $\iglobalSemantics(c) \models \safetySpecc$ and $\iglobalSemantics(c) \models \livenessSpec$). %Below, we present safety and liveness properties. \ourskip

%\para{Safety Properties.} 
Safety properties $\safetySpec$ are specified by the system designer as (Boolean combinations of) \permissible safety specifications. Such properties are invariants that must hold in every reachable state in $\iglobalSemantics$.

%\ourskip
%\para{Liveness Properties.}  
Liveness properties $\livenessSpec$ ensure that the system makes progress and eventually reacts to various environmental events. A liveness property is specified by the designer using the standard notion of \buchi automaton \cite{buchi} that accepts infinite traces in $\iglobalSemantics$ violating the property.\footnote{In fact, in \tool, the system designer can also specify liveness properties as (a restricted form of) Linear Time Logic (LTL) formulas that are then automatically translated to their \buchi automata equivalents.}



\subsection{\Counterexamples of Global Properties}
Recall that $\pcomplete$ has the global semantics $\iglobalSemantics = (\iGQ,\gq_0,\events,\iGT, \iDisGT)$, where $\iGQ$ is the set of global states, $\gq_0$ is the initial global state, 
$\events$ is the set of events,
and  $\iGT$ is the set of global transitions.
Further, recall that in the last two stages of the synthesis loop, we check if cutoff-sized system based on $\pcomplete$ is safe and live (i.e., $\isemantics \models \safetySpecc$ and $\isemantics \models \livenessSpec$). 


Similar to \counterexamples of local properties, a \counterexample $\cex$ to safety (resp. liveness) is a ``subset'' of the global semantics $\iglobalSemantics$ such that $\cex \not \models \safetySpecc$ (resp. $\cex \not \models \livenessSpec$). We say that $\cex$ is a subset of $\iglobalSemantics$, denoted $\cex \subseteq \iglobalSemantics$, when it has a subset of its enabled and disabled global transitions, i.e., $\cex = (\iGQ,\gq_0,\events,\iGT' \subseteq \iGT,\iDisGTPrime \subseteq \iDisGT)$.




\subsection{Extracting \Counterexamples to Global Properties}
A \counterexample $\cex \subseteq \iglobalSemantics$ to a safety property $\safetySpecc$ is a finite trace from the initial state $\gq_0$ to an error state $\gq_e$. %such that state $\gq_e$ violates $\safetySpec$. 
Such traces are extracted while constructing $\iglobalSemantics$.\footnote{We additionally check if the system is \emph{deadlock-free}, i.e., that $\iglobalSemantics$ does not contain any deadlock state $\gq_d$ where no event is enabled. A \counterexample $\cex$ to deadlock freedom is a trace to some deadlock state $\gq_d$ \emph{as well as} all disabled global transitions out $\gq_d$. After all, a deadlock state can be avoided if the system does not reach it, or can step out of it.}

A \counterexample $\cex \subseteq \iglobalSemantics$ to a liveness property $\livenessSpec$ is a ``lasso-shaped'' subset of the global semantics that represents an infinite, \fair, accepting trace violating $\livenessSpec$. \neww{An infinite trace is \fair if it represents a realistic infinite execution of the system as opposed to one that is merely an artifact of the non-determinism when picking which system event should be executed next.} Such $\cex$ consists of two parts: a fair, accepting \emph{cycle} in $\iglobalSemantics$, and a finite \emph{stem} from the initial state $\gq_0$ to a state in that cycle.
Identifying fair, accepting cycles and their stems is a standard technique in the literature and we defer its details to \appref{liveness}.
Note that $\cex$ \emph{additionally} contains all disabled global transitions from every state in the cycle. Intuitively, enabling any such disabled transition renders the infinite trace unfair, and hence rules out the liveness violation.


%
%
%
%
%
%
%n this document, we discuss global error/deadlock traces, what they’re composed of, and how to encode them.
%
%**Basic Observations**
%
%- A trace consists of a set of global transitions.
%- Each global transition stores, the action, the receive matrix and the send vector pair.
%- Each global transition is based on a set of local transitions, which can be persisted/retrieved when computing the receive Matrix and the send VectorPair.
%- Since the transition exists in the system, then it was deemed enabled and firable.
%- The global source state of the transition indicates where processes are located. We call these the active local states of a global state.
%- The idea is to determine the set of active local transitions that actually took place in the transition.
%- The active local transitions are simply those taken by the existing senders/receivers in the source state when the global transition happens.
%- The encoding is simply a conjunction of these.
%- When encoding a trace, we can optimize things, like we did with paths.
%
%**Deciding on active local state and transitions**
%
%Active sending transitions are easy: just persist the states used when creating the send vector-pair.
%
%Since the receive matrix is one per action, we need to check which receive transitions where actually executed. To do so, we follow this simple procedure:
%
%1. Persist a map from the set of all handling states (all states with receives) to the receive transitions.
%2. Remove the senders from the global source state.
%3. for all non-zero local states, get the corresponding receive transitions using the map in step one.
%
%**Safety Violation Trace Encoding**
%
%For some global transition $gt = q\xrightarrow{(e,M,v)} q'$ we define the function $localTrs(t)$ to return a set of active local transitions that processes use during this global transitions.  We additionally define “reachable”, “hasAction” and “endIn” the as expected. 
%
%- $\llbracket q \rrbracket = \bigwedge_{t \in localTrs(gt)} \llbracket src(t) \rrbracket$
%- $\llbracket e\mid q \rrbracket = \bigwedge_{t \in localTrs(gt)} \llbracket act(t)\mid src(t) \rrbracket$
%- $\llbracket q' \mid q, \ e\rrbracket = \bigwedge_{t \in localTrs(gt)} \llbracket dest(t) \mid src(t), \ act(t) \rrbracket$
%
%Finally, we encode a global transition in the expected way:
%
%$$
%\llbracket gt \rrbracket = \llbracket q \rrbracket \wedge \llbracket e \mid q \rrbracket \wedge \llbracket  q'\mid q,e\rrbracket =  \bigwedge_{t \in localTrs(gt)} \llbracket t \rrbracket
%$$


==> gspproc.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-1em}
\centering

\begin{tikzpicture}[->,>=stealth',auto,node distance=8cm,semithick,scale=0.49,every node/.style={transform shape}]

\tikzstyle{every edge}=[font=\fontsize{20}{0}\selectfont, draw = black, align=center]
\tikzstyle{every state}=[minimum size=1.8cm, font=\fontsize{20}{0}]

%%% node (states) definition%%%%%%

 \node[state]  (s0)                   					{$\ls_0$};
 \node[state]  (s1)  	[right = 1.6 cm of s0]    	{$\ls_1$};
 \node[state]  (s2)    	[right = 1.6 cm of s1]    	{$\ls_2$};  
 \node[state]  (s3)       [right = 1.6 cm of s2]    	{$\ls_3$};
 
%%% paths definition%%%%%%
\draw
(s0)     edge  node [above] {$a_1$}  (s1)
(s0)     edge [bend left =40]  node [above] {$a\#$}  (s2)
%(s3)     edge [bend left]  node [above] {$a_1$}  (s2)
%(s3)     edge [bend right] node [above] {$a_2$}  (s2)
(s3)     edge node [above] {$a_2$}  (s2)
(s1)    edge      [loop below]          node [left, xshift = -10] {$a\#$}     (s1)
(s2)    edge      [loop below]          node[left, xshift = -10] {$a\#$}     (s2)
(s3)    edge      [loop below]          node[left, xshift = -10] {$a\#$}     (s3)
(s3)     node [above =1.8cm,font=\fontsize{20}{0}\selectfont, xshift = -30] {$G_a=\{s_0,s_3\}$}

;
\end{tikzpicture}
\caption{An example process definition in the \hlm.}
\label{fig:gspproc}  
\vspace{-0.5em}
\end{wrapfigure}


==> synthesisAlgorithm.tex <==
% to shift the comments
\renewcommand{\Comment}[2][.33\linewidth]{\leavevmode\hfill\makebox[#1][l]{$\rhd$~#2}}

%\vspace{-1.5em}
\begin{algorithm}[t]
\footnotesize
  \SetKwFunction{synthisProc}{Synthesize}  
  \SetKwProg{myproc}{procedure}{}{}
  \myproc{\synthisProc{$\psketch, \safetySpec, \livenessSpec$}}{
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
%  \Input{A \aml program sketch, $\psketch$}  
%  \Input{\Permissible safety specification, $\safetySpec$}
%  \Input{Liveness specification, $\livenessSpec$}
%  \Output{A \chwellbehaved, \amenable, safe, and live  process $\pcomplete$, or \code{null}}
% \BlankLine
 
  $\constraints = \varnothing$ \label{line:emptyconstraints}\Comment{Empty set of constraints} 
    
  \While{true}{
    $\interpretation$ = \Call{interpret}{$\uFuns,\constraints$} \label{line:interpret} \Comment{Obtain an interpretation from a \learner}
	
    \If{$\interpretation \neq$ \code{null}} {

      $\pcomplete = $ \Call{complete}{$\psketch, \interpretation$} \label{line:completed}
      
      $\isemantics = $ \Call{buildLocalSemantics}{$\pcomplete$}
      
      $\cexPhComp$ = \Call{findPhaseCompatibilityCE}{$\isemantics$}
      \label{line:compatibility} \Comment{A \counterexample to \chwellbehavedness}
      
      \If(\label{line:notcompatible} \Comment{$\pcomplete$ is not \chwellbehaved}){$\cexPhComp  \neq$ \code{null}}{
		
		
       	$\constraints = \constraints \ \cup$ \Call{encode}{$\cexPhComp$} \label{line:encodeph}\Comment{Add constraint to eliminate $\cexPhComp$}

        \textbf{Continue} \label{line:startoverp}\Comment{Start over}
      }       
	  \BlankLine

      $\cexCutoff$ = \Call{findCutoffAmenabilityCE}{$\isemantics, \safetySpec$}
      \label{line:amenability} \Comment{A \counterexample to \amenability}
      
      \If(\label{line:notamenable} \Comment{$\pcomplete$ is not \amenable}){$\cexCutoff  \neq$ \code{null}}{
		
		
       	$\constraints = \constraints \ \cup$ \Call{encode}{$\cexCutoff$} \label{line:encodeca}\Comment{Add constraint to eliminate $\cexCutoff$}

        \textbf{Continue} \Comment{Start over}
      }       
	  \BlankLine
      
      $c$ = \Call{computeCutoff}{$\pcomplete, \safetySpec$}
      
      $\iglobalSemantics = $ \Call{buildGlobalSemantics}{$\pcomplete,c$}
       


      $\cexSafety$ = \Call{findSafetyCE}{$\iglobalSemantics,\safetySpecc$}
      \label{line:safety} \Comment{A \counterexample to safety}
      
      \If(\label{line:notsafe} \Comment{$\pcomplete$ is not safe}){$\cexSafety  \neq$ \code{null}}{
		
		
       	$\constraints = \constraints \ \cup$ \Call{encode}{$\cexSafety$} \label{line:encodes}\Comment{Add constraint to eliminate $\cexSafety$}

        \textbf{Continue} \Comment{Start over}
      }       
	  \BlankLine

      $\cexLiveness$ = \Call{findLivenessCE}{$\iglobalSemantics, \livenessSpec$}
      \label{line:liveness} \Comment{A \counterexample to liveness}
      
      \If(\label{line:notlive} \Comment{$\pcomplete$ is not live}){$\cexLiveness  \neq$ \code{null}}{
		
		
       	$\constraints = \constraints \ \cup$ \Call{encode}{$\cexLiveness$} \label{line:encodel}\Comment{Add constraint to eliminate $\cexLiveness$}

        \textbf{Continue} \Comment{Start over}
      }       
	  \BlankLine
            
      \Return $\pcomplete$ \Comment{Found a correct completion!}
      		
	}\Else{
	  \Return \code{null} \Comment{Synthesis failed, break and return \code{null}}
	}
	
  } % end of while true
} % end of procedue
\caption{Procedure for Solving \mpsp.}
\label{algo:synthAlgo}
\end{algorithm}


